Assessment of SAPT and Supermolecular EDAs Approaches for the Development of Separable and Polarizable force fields

What is the best reference quantum chemical approach to decipher the energycomponents of the total interaction energy : Symmetry-Adapted Perturbation Theory(SAPT) or Supermolecular Energy Decomposition Analysis (EDA) methods? With the rise of physically motivated polarizable force fields (polFF) grounded on these procedures, the need to answer such a question becomes critical. these procedures, the need to answer such a question becomes critical. We report a systematic and detailed assessment of three variants of SAPT (namely SAPT(2), SAPT(2+3) and SAPT(DFT) and three supermolecular EDAs approaches (ALMO, CSOV and RVS). A set of challenging, strongly bound water complexes: (H2O)2, (Zn2+)H2O and F-)H2O are used as stress-tests for these electronic structure methods. We have developed a procedure to separate the induction energy into the polarization and charge-delocalization using an infinite-order strategy based on SAPT(DFT). This paper aims to provide an overview of the capabilities and limitations, but also similarities, of SAPT and supermolecular EDAs approaches for polFF developments. Our results show that SAPT(DFT)/noS**2 and {\omega}B97X-D||ALMO are the most accurate and reliable techniques

==> Comparison_of_EDAs_HF_ref.tex <==

%\captionsetup{justification=justified,singlelinecheck=false}

\begin{figure}

\begin{center}
  %\includegraphics[bb=50 100 1000 1550, clip, scale=0.35]{misc_figs/Comparison_of_EDAs_HF_ref.pdf}
  \includegraphics[bb=100 180 1500 1550, clip, scale=0.38]{misc_figs/Comparison_of_EDAs_HF_ref+FLUOR.pdf}
\end{center}

\caption{ 
  Comparison of energy components from the supermolecular EDAs based on HF wavefunctions. Results are displayed for the water dimer, \Zn\dots\water complex and \F\dots\water complexes.
}
\label{fig:Comparison_of_EDAs_HF_ref}

\end{figure}


==> Eint_anions.tex <==

\captionsetup{justification=justified,singlelinecheck=false}

\begin{figure}

\begin{center}
 % \includegraphics[scale=0.4]{misc_figs/TOT_SAPT_SAPTDFT_DFT_anion-h2o.pdf}
  \includegraphics[viewport=70 90 1000 1190, clip, scale=0.52]{misc_figs/TOT_SAPT_SAPTDFT_DFT_anion-h2o_noS2.pdf}


\caption{ 
Comparison of the intermolecular interaction energy between DFT-based supermolecular EDAs, \sapt models, \saptdft and \ccsdt for the anionic (\F,\Cl,\OH)\dots\water complexes. The \Ssq approximation is used for the second- and third-order exchange energies in the \sapt models and \saptdftpbezssq. For \saptdftpbeznossq this approximation is present only in the \Eexdisp{2} energy.
}
\label{fig:Anions-H2O-Eint}
\end{center}
\end{figure}


==> notes-tmp.tex <==
\edits{HIGHLIGHT IN YELLOW : GRAMATICAL and MATHEMATICAL COMMENTS FROM REVIEWERS = NEED TO MAKE THE CHANGE AS THEY SUGGESTED} \\
\edits{
\begin{itemize}
\item references need to be checked
\item accuracy and grammar of the language not ok
\item the zinc issue is not clear enough, need to write step by step our argumentation (include ISA charge results ?)
\item focus only on \waterdimer, \Znwater, \Fwater to be consistent with all figures
\item we have lost our primary aim of this paper: a guide for FF developer ...perhaps to much details were written
\item emphasize our polarization model.
\item notation table added + graphical representation of the complexes
\item again results/discussion is not clear enough or perhaps to complicate to follow therefore figures will be modify as :
\end{itemize}
}
\edits{
\begin{enumerate}
    \item MERGE FIGURE 1 \& 2 AND REMOVE \Clwater and \OHwater figures (moved in the SI) : we need to be consistant with the following figures
    \item FIGURE 3 : MOVE SAPT2 panel in the SI
    \item FIGURE 4 : MOVE Tot and Disp PLOTS in the SI
    \item FIGURE 5 : DIVIDE INTO 2 FIGURES POL AND CD
    \item[] + sublabels A, B, C ... will be added
\end{enumerate}
}

